OpenAirLink: Reproducible Wireless Channel Emulation using Software Defined Radios

This paper presents OpenAirLink(OAL), an open-source channel emulator for reproducible testing of wireless scenarios. OAL is implemented on off-the-shelf software-defined radios (SDR) and presents a smaller-scale alternative to expensive commercially available channel emulators. Path loss and propagation delay are the fundamental aspects of emulating a wireless channel. OAL provides a simple method to change these aspects in real-time. The emulator is implemented using a finite impulse response (FIR) filter. The FIR filter is written in Verilog and flashed on the SDRs Field Programmable Gate Array (FPGA). Most processing transpires on the FPGA, so OAL does not require high-performance computing hardware and SDRs. We validate the performance of OAL and demonstrate the utility of such a channel emulation tool using two examples. We believe that open-source channel emulators such as OAL can make reproducible wireless experiments accessible to many researchers in the scientific community.

==> Images/tikz/fig-chan-step.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=2.562in,
at={(0in,0in)},
scale only axis,
xmin=-1,
xmax=31,
xlabel style={font=\color{white!15!black}},
xlabel={$G dB$},
ymin=0,
ymax=0.009,
ylabel style={font=\color{white!15!black}},
ylabel={$\Delta G$dB},
axis background/.style={fill=white},
legend style={at={(0.03,0.97)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot[ycomb, color=blue, mark=asterisk, mark options={solid, blue}] table[row sep=crcr] {%
-0	0.000265076360379612\\
0.999886827458977	0.000297416139255859\\
1.99991766159762	0.00033370688434409\\
3.00009717302558	0.000374432143093172\\
3.99982325834229	0.000420105421380529\\
5.00011228629973	0.000471380329427248\\
6.00021266695863	0.000528901789662662\\
7.00028560654258	0.000593440347175776\\
7.99985195410919	0.000665815004585134\\
9.00012725042659	0.000747076905640077\\
9.99986186381193	0.000838204067050623\\
10.9999956273088	0.000940489377570136\\
11.9996815890644	0.001055201317955\\
12.9995471695947	0.00118392825618706\\
13.999835297947	0.00132842236828011\\
14.999833261031	0.00149050015604983\\
16.0003671709329	0.00167245396455283\\
17.0008666172397	0.00187661006197451\\
18.0002545651151	0.00210541502377661\\
18.9988610254567	0.00236190066392547\\
19.9992047951865	0.00265015704208988\\
21.0010765938656	0.00297411050262818\\
21.9992502606493	0.00333623573837241\\
22.998973925016	0.00374311130036151\\
24.0019240902882	0.00420115589233213\\
24.9982269184525	0.00471162997073402\\
26.0012705671655	0.0052882130327953\\
26.9979120883865	0.00593095935510337\\
28.003181794916	0.00665840556796695\\
28.997139328265	0.00746531170842531\\
30.0015385146497	0.00838001959653439\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
-1	0\\
31	0\\
};
\addlegendentry{FIR only}

\addplot[ycomb, color=red, mark=o, mark options={solid, red}] table[row sep=crcr] {%
0	0.000265076360379612\\
0.999886827458977	0.000297416139255859\\
1.99991766159762	0.00033370688434409\\
3.00009717302558	0.000374432143093172\\
3.99982325834229	0.000420105421380529\\
5.00011228629973	0.000471380329427248\\
6.00021266695863	0.000528901789662662\\
6.99998888130084	0.000296715105434175\\
7.99985195410919	0.000332913882030837\\
9.00012725042659	0.000373546484868655\\
9.99986186381193	0.000419112144551456\\
10.9999956273088	0.000470257418054978\\
12.0002092377988	0.000527648734363887\\
13.0001391942439	0.000296017368625731\\
13.999835297947	0.000332124639676498\\
14.999833261031	0.000372649018143533\\
15.9999490272506	0.000418123553553757\\
16.9999282615279	0.000469139843915568\\
18.0002545651151	0.000526401602419828\\
19.0000422166788	0.000295312864900462\\
19.9998674608086	0.000331339130600175\\
20.9999611830851	0.000371771765335085\\
22.0000845198477	0.000417139615306476\\
22.9999099549364	0.000468027569047554\\
23.9998232583423	0.000525128601959646\\
24.9999944388191	0.000294611706569001\\
25.9999482120381	0.000330557328377458\\
27.0001372426546	0.000370898633105282\\
27.9998519541092	0.000416140358832613\\
28.9999404751761	0.000466920555848148\\
29.999966645008	0.00052389334061309\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
-1	0\\
31	0\\
};
\addlegendentry{with Bit Shift}

\end{axis}
\end{tikzpicture}%

==> Images/tikz/fig-emu-delay.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.306in,
height=2.666in,
at={(0.0in,0.0in)},
scale only axis,
xmin=-2,
xmax=42,
xlabel style={font=\color{white!15!black}},
xlabel={Delayed Taps},
ymin=-10,
ymax=215,
ylabel style={font=\color{white!15!black}},
ylabel={Time [ns]},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.03,0.97)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
0	0\\
4	19.1666666666651\\
8	40.2777777777757\\
12	69.9999999999989\\
16	79.7222222222227\\
20	109.166666666667\\
24	119.166666666665\\
28	139.166666666666\\
32	169.72222222222\\
36	178.888888888886\\
40	208.888888888889\\
};
\addlegendentry{Emulator}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
0	0\\
4	20.0000000000000\\
8	40.0000000000000\\
12	60.0000000000000\\
16	80.0000000000000\\
20	100.000000000000\\
24	120.000000000000\\
28	140.000000000000\\
32	160.000000000000\\
36	180.000000000000\\
40	200.000000000000\\
};
\addlegendentry{Spirent Vertex Emulator}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0	0\\
4	20\\
8	40\\
12	60\\
16	80\\
20	100\\
24	120\\
28	140\\
32	160\\
36	180\\
40	200\\
};
\addlegendentry{Theoretical Delay}

\end{axis}
\end{tikzpicture}%

==> Maths/Algorithms/param_loader.tex <==
\begin{algorithm}
\caption{Loading and Writing Channel Parameters}
\begin{algorithmic}[1]
\Function{ProcessCSV}{$filename, timestamp$}
    \State $unix\_timestamp \gets \text{Unix timestamp of } timestamp$
    \State $rows \gets \text{ReadCSV}(filename)$
    \For{$row$ \textbf{in} $rows$}
        \For{$i \gets 1$ \textbf{to} $\text{length}(row)$}
            \If{$i > unix\_timestamp$}
                \State $row[i] \gets row[i] \% \text{ some\_value}$
            \EndIf
        \EndFor
        \State \textbf{do something with} $row$
    \EndFor
\EndFunction
\end{algorithmic}
\end{algorithm}
